CircuitVAE: Efficient and Scalable Latent Circuit Optimization

Automatically designing fast and space-efficient digital circuits is challenging because circuits are discrete, must exactly implement the desired logic, and are costly to simulate. We address these challenges with CircuitVAE, a search algorithm that embeds computation graphs in a continuous space and optimizes a learned surrogate of physical simulation by gradient descent. By carefully controlling overfitting of the simulation surrogate and ensuring diverse exploration, our algorithm is highly sample-efficient, yet gracefully scales to large problem instances and high sample budgets. We test CircuitVAE by designing binary adders across a large range of sizes, IO timing constraints, and sample budgets. Our method excels at designing large circuits, where other algorithms struggle: compared to reinforcement learning and genetic algorithms, CircuitVAE typically finds 64-bit adders which are smaller and faster using less than half the sample budget. We also find CircuitVAE can design state-of-the-art adders in a real-world chip, demonstrating that our method can outperform commercial tools in a realistic setting.

==> sections/limitations_impact.tex <==
\section{Limitations and Broader Impact}
One limitation of our method is its dependence on a netlist generator, which allows us to compactly represent circuit designs as graphs our autoencoder can ingest.
While parallel prefix trees provide this representation for binary adders, other types of circuits may require different graph descriptions (e.g. Wallace trees \citep{wallace_trees} for multipliers) or have no straightforward graph description (e.g. dense combinational logic).
Another limitation is its dependence on an initial search algorithm used to generate the initial training data, which we explore in \autoref{subsec:ablations}.
Future work could explore extending CircuitVAE to other circuit types by changing the netlist generator or reduce its dependence on initial data.

As \citet{dualuse} show, combinatorial optimization has potential for misuse by bad actors.
While logic optimization offers few such possibilities, several of the techniques we discuss could apply to other domains such as drug design.
On balance, we believe that the benefits of accelerating automated design outweigh the potential drawbacks.
